Testing Scientific Software: A Systematic Literature Review

Context: Scientific software plays an important role in critical decision making, for example making weather predictions based on climate models, and computation of evidence for research publications. Recently, scientists have had to retract publications due to errors caused by software faults. Systematic testing can identify such faults in code. Objective: This study aims to identify specific challenges, proposed solutions, and unsolved problems faced when testing scientific software. Method: We conducted a systematic literature survey to identify and analyze relevant literature. We identified 62 studies that provided relevant information about testing scientific software. Results: We found that challenges faced when testing scientific software fall into two main categories: (1) testing challenges that occur due to characteristics of scientific software such as oracle problems and (2) testing challenges that occur due to cultural differences between scientists and the software engineering community such as viewing the code and the model that it implements as inseparable entities. In addition, we identified methods to potentially overcome these challenges and their limitations. Finally we describe unsolved challenges and how software engineering researchers and practitioners can help to overcome them. Conclusions: Scientific software presents special challenges for testing. Specifically, cultural differences between scientist developers and software engineers, along with the characteristics of the scientific software make testing more difficult. Existing techniques such as code clone detection can help to improve the testing process. Software engineers should consider special challenges posed by scientific software such as oracle problems when developing testing techniques.

==> refs/ReferenceListFromPrimaryPapers_selectedByReading <==
% This file was created with JabRef 2.9.2.
% Encoding: UTF-8

@CONFERENCE{BagnaraCGG13,
  author = {Roberto Bagnara and Matthieu Carlier and Roberta Gori and Arnaud
	Gotlieb},
  title = {Symbolic Path-Oriented Test Data Generation for Floating-Point Programs},
  booktitle = {Proceedings of the 6th IEEE International Conference on Software
	Testing, Verification and Validation},
  year = {In Press},
  address = {Luxembourg City, Luxembourg},
  organization = {IEEE Press},
  publisher = {IEEE Press},
  abstract = {Verifying critical numerical software involves the generation of test
	data for floating-point intensive programs. As the symbolic execution
	of floating-point computations presents significant difficulties,
	existing approaches usually resort to random or search-based test
	data generation. However, without symbolic reasoning, it is almost
	impossible to generate test inputs that execute many paths with floating-point
	computations. Moreover, constraint solvers over the reals or the
	rationals do not handle the rounding errors. In this paper, we present
	a new version of FPSE, a symbolic evaluator for C program paths,
	that specifically addresses this problem. The tool solves path conditions
	containing floating-point computations by using correct and precise
	projection functions. This version of the tool exploits an essential
	filtering property based on the representation of floating-point
	numbers that makes it suitable to generate path-oriented test inputs
	for complex paths characterized by floating- point intensive computations.
	The paper reviews the key implementation choices in FPSE and the
	labeling search heuristics we selected to maximize the benefits of
	enhanced filtering. Our experimental results show that FPSE can generate
	correct test inputs for selected paths containing several hundreds
	of iterations and thousands of executable floating-point statements
	on a standard machine: this is currently outside the scope of any
	other symbolic-execution test data generator tool.},
  attachments = {http://bugseng.com/sites/bugseng.com/files/BagnaraCGG13ICST.pdf},
  keywords = {floating-point, IEEE 754, testing, verification},
  owner = {upuleegk},
  timestamp = {2013.03.15}
}

@INPROCEEDINGS{Carver:2007:SDE:1248820.1248886,
  author = {Carver, Jeffrey C. and Kendall, Richard P. and Squires, Susan E.
	and Post, Douglass E.},
  title = {Software Development Environments for Scientific and Engineering
	Software: A Series of Case Studies},
  booktitle = {Proceedings of the 29th international conference on Software Engineering},
  year = {2007},
  series = {ICSE '07},
  pages = {550--559},
  address = {Washington, DC, USA},
  publisher = {IEEE Computer Society},
  acmid = {1248886},
  doi = {10.1109/ICSE.2007.77},
  isbn = {0-7695-2828-7},
  numpages = {10},
  owner = {upuleegk},
  timestamp = {2013.03.15},
  url = {http://dx.doi.org/10.1109/ICSE.2007.77}
}

@INPROCEEDINGS{1045022,
  author = {Chen, T.Y. and Jianqiang Feng and Tse, T. H.},
  title = {Metamorphic testing of programs on partial differential equations:
	a case study},
  booktitle = {Computer Software and Applications Conference, 2002. COMPSAC 2002.
	Proceedings. 26th Annual International},
  pages = {327-333},
  doi = {10.1109/CMPSAC.2002.1045022},
  issn = {0730-3157},
  keywords = {elliptic equations;mathematics computing;partial differential equations;program
	testing;Dirichlet boundary conditions;case study;elliptic partial
	differential equation;metamorphic program testing;numerical programs;oracle
	problem;Application software;Biomedical engineering;Boundary conditions;Computer
	aided software engineering;Mission critical systems;Packaging;Partial
	differential equations;Software libraries;Software standards;Software
	testing},
  owner = {upuleegk},
  timestamp = {2013.03.15}
}

@ARTICLE{journals/bmcbi/ChenHLX09,
  author = {Chen, Tsong Yueh and Ho, Joshua W. K. and Liu, Huai and Xie, Xiaoyuan},
  title = {An innovative approach for testing bioinformatics programs using
	metamorphic testing.},
  journal = {BMC Bioinformatics},
  year = {2009},
  volume = {10},
  added-at = {2009-08-21T00:00:00.000+0200},
  biburl = {http://www.bibsonomy.org/bibtex/2a40f63ff326b0560f84475c7a0c840b2/dblp},
  date = {2009-08-21},
  description = {dblp},
  ee = {http://dx.doi.org/10.1186/1471-2105-10-24},
  interhash = {cb07768529c31b0c92fbc9d3acdf5363},
  intrahash = {a40f63ff326b0560f84475c7a0c840b2},
  keywords = {dblp},
  owner = {upuleegk},
  timestamp = {2009-08-21T00:00:00.000+0200},
  url = {http://dblp.uni-trier.de/db/journals/bmcbi/bmcbi10.html#ChenHLX09}
}

@INPROCEEDINGS{Davis:1981:PNP:800175.809889,
  author = {Davis, Martin D. and Weyuker, Elaine J.},
  title = {Pseudo-oracles for non-testable programs},
  booktitle = {Proceedings of the ACM '81 conference},
  year = {1981},
  series = {ACM '81},
  pages = {254--257},
  address = {New York, NY, USA},
  publisher = {ACM},
  acmid = {809889},
  doi = {10.1145/800175.809889},
  isbn = {0-89791-049-4},
  numpages = {4},
  owner = {upuleegk},
  timestamp = {2013.03.15},
  url = {http://doi.acm.org/10.1145/800175.809889}
}

@ARTICLE{4476223,
  author = {Hochstein, L. and Basili, V.R.},
  title = {The ASC-Alliance Projects: A Case Study of Large-Scale Parallel Scientific
	Code Development},
  journal = {Computer},
  year = {March},
  volume = {41},
  pages = {50-58},
  number = {3},
  doi = {10.1109/MC.2008.101},
  issn = {0018-9162},
  keywords = {large-scale systems;parallel machines;software engineering;ASC-Alliance
	projects;computational science software projects;computational scientists;large
	scale parallel scientific code development;parallel machines;software
	development;Computational modeling;Concurrent computing;Containers;Electric
	shock;Fires;Large-scale systems;Parallel machines;Programming;Rockets;Solid
	modeling;computing methodologies;scientific code development;simulation;software
	engineering},
  owner = {upuleegk},
  timestamp = {2013.03.15}
}

@ARTICLE{DBLP:journals/bmcbi/KaneHCMKB06,
  author = {David W. Kane and Moses M. Hohman and Ethan G. Cerami and Michael
	W. McCormick and Karl F. Kuhlmman and Jeff A. Byrd},
  title = {Agile methods in biomedical software development: a multi-site experience
	report},
  journal = {BMC Bioinformatics},
  year = {2006},
  volume = {7},
  pages = {273},
  bibsource = {DBLP, http://dblp.uni-trier.de},
  ee = {http://dx.doi.org/10.1186/1471-2105-7-273},
  owner = {upuleegk},
  timestamp = {2013.03.15}
}

@INPROCEEDINGS{Mayer05ontesting,
  author = {Johannes Mayer and Abteilung Angewandte Informationsverarbeitung
	and Universität Ulm},
  title = {On testing image processing applications with statistical methods},
  booktitle = {In Software Engineering (SE 2005), Lecture Notes in Informatics},
  year = {2005},
  pages = {69--78},
  owner = {upuleegk},
  timestamp = {2013.03.15}
}

@MISC{Murphy_anapproach,
  author = {Christian Murphy and Gail Kaiser and Marta Arias},
  title = {An Approach to Software Testing of Machine Learning Applications},
  owner = {upuleegk},
  timestamp = {2013.03.15}
}

@MISC{Murphy_propertiesof,
  author = {Christian Murphy and Gail Kaiser and Lifeng Hu and Leon Wu},
  title = {Properties of Machine Learning Applications for Use in Metamorphic
	Testing},
  owner = {upuleegk},
  timestamp = {2013.03.15}
}

@INPROCEEDINGS{5069157,
  author = {Parker, S. and Willenbring, J.M.},
  title = {Barely sufficient software engineering: 10 practices to improve your
	CSE software},
  booktitle = {Software Engineering for Computational Science and Engineering, 2009.
	SECSE '09. ICSE Workshop on},
  year = {May},
  pages = {15-21},
  doi = {10.1109/SECSE.2009.5069157},
  keywords = {software engineering;CSE software teams;Trilinos project;computational
	science and engineering;formal methods;formal software engineering;Application
	software;Automotive engineering;Laboratories;Programming;Research
	and development;Software algorithms;Software engineering;Software
	libraries;Software quality;US Department of Energy},
  owner = {upuleegk},
  timestamp = {2013.03.15}
}

@INPROCEEDINGS{oro17671,
  author = {Judith Segal},
  title = {Scientists and software engineers: A tale of two cultures},
  booktitle = {PPIG 2008: Proceedings of the 20th Annual Meeting of the Pschology
	of Programming Interest Group},
  year = {2008},
  editor = {Jim Buckley and John Rooksby and Roman Bednarik},
  address = {Lancaster, UK},
  publisher = {Lancaster University},
  note = {Proceedings: 20th annual meeting of the Psychology of Programming
	Interest Group; Lancaster, United Kingdom; September 10-12 2008},
  abstract = {The two cultures of the title are those observed in my field studies:
	the culture of scientists (financial mathematicians, earth and planetary
	scientists, and molecular biologists) developing their own software,
	and the culture of software engineers developing scientific software.
	In this paper, I shall describe some problems arising when scientists
	and software engineers come together to develop scientific software
	and discuss how these problems may be ascribed to their two different
	cultures.},
  keywords = {POP-I C Ill-defined problems; POP-II A End-users; POP {\"i}??II C
	Working practices; POP-V B Case studies;},
  owner = {upuleegk},
  timestamp = {2013.03.15},
  url = {http://oro.open.ac.uk/17671/}
}

@INPROCEEDINGS{oro17674,
  author = {Judith Segal},
  title = {Some problems of professional end user developers},
  booktitle = {Visual Languages and Human-Centric Computing},
  year = {2007},
  editor = {Philip Cox and John Hosking},
  volume = {VL/HCC},
  pages = {111--118},
  address = {Los Alamitos, Ca, USA,},
  month = {September},
  publisher = {IEEE Computer Society/Conference Publishing Services},
  abstract = {By the term 'professional end user developers' we mean people such
	as research scientists who work in highly technical, knowledge-rich
	domains and who develop software in order to further their professional
	goals. In common with other end user developers, professional end
	user developers do not describe themselves as software engineers
	and have no formal training in software engineering. They differ
	from most other end user developers, however, in that learning programming
	languages rarely presents them with any problem. In this paper, drawing
	on data from field studies of different groups of professional end
	users, we examine the problems that such people face in meeting the
	demands of software development given the culture in which they work
	and their normal development practice. Understanding these problems
	is an essential prerequisite to developing tools, techniques etcetera
	to support professional end user development.},
  keywords = {software development management; non-controlled indexing; knowledge-rich
	domains; learning programming languages; professional end user developers;
	software development; software engineering},
  owner = {upuleegk},
  timestamp = {2013.03.15},
  url = {http://oro.open.ac.uk/17674/}
}

@ARTICLE{oro18494,
  author = {Judith Segal},
  title = {Software development cultures and cooperation problems: a field study
	of the early stages of development of software for a scientific community},
  journal = {Computer Supported Cooperative Work},
  year = {2009},
  volume = {18},
  pages = {581--606},
  number = {5-6},
  month = {December/Winter},
  abstract = {In earlier work, I identified a particular class of end-user developers,
	who include scientists and whom I term 'professional end-user developers',
	as being of especial interest. Here, I extend this work by articulating
	a culture of professional end-user development, and illustrating
	by means of a field-study how the influence of this culture causes
	cooperation problems in an inter-disciplinary team developing a software
	system for a scientific community. My analysis of the field study
	data is informed by some recent literature on multi-national work
	cultures. Whilst acknowledging that viewing a scientific development
	through a lens of software development culture does not give a full
	picture, I argue that it nonetheless provides deep insights.},
  keywords = {community software development; cooperation; field study; scientific
	software development; software development culture; professional
	end-user developers},
  owner = {upuleegk},
  timestamp = {2013.03.15},
  url = {http://oro.open.ac.uk/18494/}
}

@ARTICLE{1196317,
  author = {Wood, W.A. and Kleb, W.L.},
  title = {Exploring XP for scientific research},
  journal = {Software, IEEE},
  year = {May-June},
  volume = {20},
  pages = {30-36},
  number = {3},
  doi = {10.1109/MS.2003.1196317},
  issn = {0740-7459},
  keywords = {aerospace computing;programming;project engineering;software engineering;Extreme
	Programming;NASA Langley Research Center;XP practices;agile programming;cultural
	conflicts;mission-critical software;pair programming;research projects;Flowcharts;Government;ISO;Missiles;NASA;Programming
	profession;Prototypes;Software prototyping;Software quality;Testing},
  owner = {upuleegk},
  timestamp = {2013.03.15}
}

@comment{jabref-meta: selector_review:}

@comment{jabref-meta: selector_publisher:}

@comment{jabref-meta: selector_author:}

@comment{jabref-meta: selector_journal:}

@comment{jabref-meta: selector_keywords:}



==> refs/SysLitReview_selectedByReading <==
% This file was created with JabRef 2.9.2.
% Encoding: UTF-8

@ARTICLE{ABACKERLI2010,
  author = {Abackerli, Alvaro Jos\~A\copyright AND Pereira, Paulo Henrique AND
	Cal\~A\'{}nego Jr., Nivaldi},
  title = {{A case study on testing CMM uncertainty simulation software (VCMM)}},
  journal = {{Journal of the Brazilian Society of Mechanical Sciences and Engineering}},
  year = {2010},
  volume = {32},
  pages = {8 - 14},
  month = {03},
  crossref = {10.1590/S1678-58782010000100002},
  issn = {1678-5878},
  language = {en},
  owner = {upuleegk},
  publisher = {scielo},
  timestamp = {2013.02.28},
  url = {http://www.scielo.br/scielo.php?script=sci_arttext&pid=S1678-58782010000100002&nrm=iso}
}

@ARTICLE{4548407,
  author = {Ackroyd, K.S. and Kinder, S.H. and Mant, G.R. and Miller, M.C. and
	Ramsdale, C.A. and Stephenson, P.C.},
  title = {Scientific Software Development at a Research Facility},
  journal = {Software, IEEE},
  year = {2008},
  volume = {25},
  pages = {44 -51},
  number = {4},
  month = {july-aug. },
  doi = {10.1109/MS.2008.93},
  issn = {0740-7459},
  keywords = {Computer science;Councils;Data acquisition;Data engineering;Laboratories;Light
	sources;Programming;Software development management;Synchrotron radiation;X-rays;data
	acquisition;natural sciences computing;research and development;software
	engineering;Daresbury Laboratory;data acquisition software;experiment
	control;research facility;scientific research;scientific software
	development;Requirements;management of computing and information
	systems;people management;physical sciences and engineering;project
	management;software construction;software engineering;specifications;},
  owner = {upuleegk},
  timestamp = {2013.03.01}
}

@TECHREPORT{CaverWhat2011,
  author = {Carver, Jeffrey, Roscoe Bartlett, Dustin Heaton and Lorin Hochstein},
  title = {What Scientists and Engineers Think They Know About Software Engineering:
	A Survey},
  institution = {Sandia National Laboratories},
  year = {2011},
  number = {SAND2011-2196},
  owner = {upuleegk},
  timestamp = {2013.02.14}
}

@ARTICLE{5999647,
  author = {Clune, T.L. and Rood, R.B.},
  title = {Software Testing and Verification in Climate Model Development},
  journal = {Software, IEEE},
  year = {2011},
  volume = {28},
  pages = {49 -55},
  number = {6},
  month = {nov.-dec. },
  doi = {10.1109/MS.2011.117},
  issn = {0740-7459},
  keywords = {Atmospheric measurements;Atmospheric modeling;Computational modeling;Global
	warming;Meteorology;Numerical models;Software development;climatology;digital
	simulation;geophysics computing;program diagnostics;program testing;program
	verification;atmospheric process;climate model development;climate
	simulation;computer infrastructure;computing resources;defect detection;defect
	diagnosis;defect isolation;parallel clusters;software testing;software
	verification;system-level regression test;verification process;program
	verification;software engineering;testing and debugging;testing strategies;},
  owner = {upuleegk},
  timestamp = {2013.02.28}
}

@ARTICLE{Cox1999339,
  author = {M.G. Cox and P.M. Harris},
  title = {Design and use of reference data sets for testing scientific software},
  journal = {Analytica Chimica Acta},
  year = {1999},
  volume = {380},
  pages = {339 - 351},
  number = {2â€“3},
  doi = {10.1016/S0003-2670(98)00481-4},
  issn = {0003-2670},
  keywords = {Reference data sets},
  owner = {upuleegk},
  timestamp = {2013.02.28},
  url = {http://www.sciencedirect.com/science/article/pii/S0003267098004814}
}

@INCOLLECTION{DahlgrenPerformance2007,
  author = {Dahlgren, TamaraL.},
  title = {Performance-Driven Interface Contract Enforcement for Scientific
	Components},
  booktitle = {Component-Based Software Engineering},
  publisher = {Springer Berlin Heidelberg},
  year = {2007},
  editor = {Schmidt, HeinzW. and Crnkovic, Ivica and Heineman, GeorgeT. and Stafford,
	JudithA.},
  volume = {4608},
  series = {Lecture Notes in Computer Science},
  pages = {157-172},
  doi = {10.1007/978-3-540-73551-9_11},
  isbn = {978-3-540-73550-2},
  owner = {upuleegk},
  timestamp = {2013.02.28},
  url = {http://dx.doi.org/10.1007/978-3-540-73551-9_11}
}

@INPROCEEDINGS{Dahlgren:2005:ISS:1145319.1145341,
  author = {Dahlgren, Tamara L. and Devanbu, Premkumar T.},
  title = {Improving scientific software component quality through assertions},
  booktitle = {Proceedings of the second international workshop on Software engineering
	for high performance computing system applications},
  year = {2005},
  series = {SE-HPCS '05},
  pages = {73--77},
  address = {New York, NY, USA},
  publisher = {ACM},
  acmid = {1145341},
  doi = {10.1145/1145319.1145341},
  isbn = {1-59593-117-1},
  keywords = {Babel, SIDL, constrained enforcement, interface assertions},
  location = {St. Louis, Missouri},
  numpages = {5},
  owner = {upuleegk},
  timestamp = {2013.02.28},
  url = {http://doi.acm.org/10.1145/1145319.1145341}
}

@ARTICLE{Drake:2005:OSD:1093627.1093634,
  author = {Drake, John B. and Jones, Philip W. and Carr,Jr., George R.},
  title = {Overview of the Software Design of the Community Climate System Model},
  journal = {Int. J. High Perform. Comput. Appl.},
  year = {2005},
  volume = {19},
  pages = {177--186},
  number = {3},
  month = aug,
  acmid = {1093634},
  address = {Thousand Oaks, CA, USA},
  doi = {10.1177/1094342005056094},
  issn = {1094-3420},
  issue_date = {August 2005},
  keywords = {Parallel clusters, multiphysics simulation},
  numpages = {10},
  owner = {upuleegk},
  publisher = {Sage Publications, Inc.},
  timestamp = {2013.02.28},
  url = {http://dx.doi.org/10.1177/1094342005056094}
}

@ARTICLE{6241365,
  author = {Dubois, P.F.},
  title = {Testing Scientific Programs},
  journal = {Computing in Science Engineering},
  year = {2012},
  volume = {14},
  pages = {69 -73},
  number = {4},
  month = {july-aug. },
  doi = {10.1109/MCSE.2012.84},
  issn = {1521-9615},
  keywords = {Automation;Biomechanics;Collaborative work;Open source software;Program
	processors;Programming;Scientific computing;Simulation;Software engineering;automatic
	test software;program testing;programming languages;public domain
	software;software tools;ATS;Python-based tool;automated testing system;open
	source;scientific programs testing;scientific simulations;subject-matter
	experts;Automation;Biomechanics;Collaborative work;Open source software;Program
	processors;Programming;Scientific computing;Simulation;Software engineering;computer
	simulations;scientific computing;scientific programming;software
	testing;team development;},
  owner = {upuleegk},
  timestamp = {2013.02.28}
}

@INPROCEEDINGS{Easterbrook:2010:CCG:1882362.1882383,
  author = {Easterbrook, Steve M.},
  title = {Climate change: a grand software challenge},
  booktitle = {Proceedings of the FSE/SDP workshop on Future of software engineering
	research},
  year = {2010},
  series = {FoSER '10},
  pages = {99--104},
  address = {New York, NY, USA},
  publisher = {ACM},
  acmid = {1882383},
  doi = {10.1145/1882362.1882383},
  isbn = {978-1-4503-0427-6},
  keywords = {climate change},
  location = {Santa Fe, New Mexico, USA},
  numpages = {6},
  owner = {upuleegk},
  timestamp = {2013.02.28},
  url = {http://doi.acm.org/10.1145/1882362.1882383}
}

@ARTICLE{5337646,
  author = {Easterbrook, Steve M. and Johns, Timothy C.},
  title = {Engineering the Software for Understanding Climate Change},
  journal = {Computing in Science Engineering},
  year = {2009},
  volume = {11},
  pages = {65 -74},
  number = {6},
  month = {nov.-dec. },
  doi = {10.1109/MCSE.2009.193},
  issn = {1521-9615},
  keywords = {Computational modeling;Earth;High performance computing;Open source
	software;Physics computing;Programming;Software engineering;Software
	maintenance;Software performance;Software quality;Software development
	processes;agile;climate models;open source;testing;validation;},
  owner = {upuleegk},
  timestamp = {2013.02.28}
}

@ARTICLE{5235131,
  author = {Eddins, S},
  title = {Automated Software Testing for MATLAB},
  journal = {Computing in Science Engineering},
  year = {2010},
  volume = {PP},
  pages = {1},
  number = {99},
  month = { },
  doi = {10.1109/MCSE.2009.160},
  issn = {1521-9615},
  keywords = {Automatic testing;Computer bugs;Data processing;MATLAB;Packaging;Programming
	profession;Reliability engineering;Software performance;Software
	testing;Writing;C.1.2.g Parallel processors;Computer aided software
	engineering;D.2.5.k Testing strategies;D.2.5.o Test execution;D.2.5.r
	Testing tools;Data mining;E.1.d Graphs and networks;F.2.2.b Computations
	on discrete structures;F.2.2.c Geometrical problems and computations;G.1.0.g
	Parallel algorithms;G.2.2.a Graph algorithms;G.2.2.d Network problems;I.4.10.a
	Hierarchical;I.4.10.b Morphological;I.4.10.c Multidimensional;I.4.3.a
	Filtering;I.4.3.b Geometric correction;I.4.3.c Grayscale manipulation;I.4.6.a
	Edge and feature detection;I.4.6.e Region growing;I.4.7.b Invariants;I.4.7.f
	Texture;MATLAB;Monitoring;NA;Testing;partitioning;},
  owner = {upuleegk},
  timestamp = {2013.03.01}
}

@ARTICLE{gmd-4-435-2011,
  author = {Farrell, P. E. and Piggott, M. D. and Gorman, G. J. and Ham, D. A.
	and Wilson, C. R. and Bond, T. M.},
  title = {Automated continuous verification for numerical simulation},
  journal = {Geoscientific Model Development},
  year = {2011},
  volume = {4},
  pages = {435--449},
  number = {2},
  doi = {10.5194/gmd-4-435-2011},
  owner = {upuleegk},
  timestamp = {2013.02.28},
  url = {http://www.geosci-model-dev.net/4/435/2011/}
}

@INPROCEEDINGS{Hannay:2009:SDU:1556904.1556928,
  author = {Hannay, Jo Erskine and MacLeod, Carolyn and Singer, Janice and Langtangen,
	Hans Petter and Pfahl, Dietmar and Wilson, Greg},
  title = {How do scientists develop and use scientific software?},
  booktitle = {Proceedings of the 2009 ICSE Workshop on Software Engineering for
	Computational Science and Engineering},
  year = {2009},
  series = {SECSE '09},
  pages = {1--8},
  address = {Washington, DC, USA},
  publisher = {IEEE Computer Society},
  acmid = {1556928},
  doi = {10.1109/SECSE.2009.5069155},
  isbn = {978-1-4244-3737-5},
  numpages = {8},
  owner = {upuleegk},
  timestamp = {2013.02.28},
  url = {http://dx.doi.org/10.1109/SECSE.2009.5069155}
}

@ARTICLE{609829,
  author = {Hatton, L.},
  title = {The T experiments: errors in scientific software},
  journal = {Computational Science Engineering, IEEE},
  year = {1997},
  volume = {4},
  pages = {27 -38},
  number = {2},
  month = {apr-jun},
  doi = {10.1109/99.609829},
  issn = {1070-9924},
  keywords = {Aerodynamics;Application software;Area measurement;Computer industry;Fault
	detection;Floating-point arithmetic;Laboratories;Radio access networks;Software
	measurement;Software testing;computer science education;software
	engineering;T experiments;scientific software;software codes;software
	engineering practices;},
  owner = {upuleegk},
  timestamp = {2013.02.28}
}

@ARTICLE{328993,
  author = {Hatton, L. and Roberts, A.},
  title = {How accurate is scientific software?},
  journal = {Software Engineering, IEEE Transactions on},
  year = {1994},
  volume = {20},
  pages = {785 -797},
  number = {10},
  month = {oct},
  doi = {10.1109/32.328993},
  issn = {0098-5589},
  keywords = {Arithmetic;Computer industry;Computer languages;Data processing;Feedback;Geoscience;Packaging;Programming;Software
	standards;Standards development;geophysics computing;programming;seismology;software
	packages;software quality;Fortran;N-version programming experiment;input
	dataset;large commercial packages;mathematical algorithms;programming
	language;quality assurance;quality standards;scientific computation;scientific
	software;seismic data processing;seismic data processing industry;software
	development;},
  owner = {upuleegk},
  timestamp = {2013.02.28}
}

@INPROCEEDINGS{4135253,
  author = {Heroux, Michael A. and Willenbring, James. M. and Phenow, Michael
	N.},
  title = {Improving the Development Process for CSE Software},
  booktitle = {Parallel, Distributed and Network-Based Processing, 2007. PDP '07.
	15th EUROMICRO International Conference on},
  year = {2007},
  pages = {11 -17},
  month = {feb.},
  doi = {10.1109/PDP.2007.51},
  issn = {1066-6192},
  keywords = {Application software;Cultural differences;Electronic mail;Mathematical
	programming;Packaging;Software algorithms;Software quality;Software
	tools;Technological innovation;Writing;formal verification;software
	development management;software metrics;software quality;software
	tools;CSE software;Trilinos Project;computational science and engineering;engineering
	programming;scientific programming;software development models;software
	processes;software quality assurance;system development;verifiable
	software quality;},
  owner = {upuleegk},
  timestamp = {2013.02.28}
}

@INPROCEEDINGS{5069163,
  author = {Hook, D. and Kelly, D.},
  title = {Testing for trustworthiness in scientific software},
  booktitle = {Software Engineering for Computational Science and Engineering, 2009.
	SECSE '09. ICSE Workshop on},
  year = {2009},
  pages = {59 -64},
  month = {may},
  doi = {10.1109/SECSE.2009.5069163},
  keywords = {Computational modeling;Computer errors;Computer languages;Educational
	institutions;Genetic mutations;Mathematical model;Performance evaluation;Software
	engineering;Software standards;Software testing;program testing;software
	engineering;oracles;scientific software testing;software engineering;standard
	testing;trustworthiness;},
  owner = {upuleegk},
  timestamp = {2013.02.28}
}

@ARTICLE{Howden:1980:ASV:357103.357107,
  author = {Howden, W. E.},
  title = {Applicability of Software Validation Techniques to Scientific Programs},
  journal = {ACM Trans. Program. Lang. Syst.},
  year = {1980},
  volume = {2},
  pages = {307--320},
  number = {3},
  month = jul,
  acmid = {357107},
  address = {New York, NY, USA},
  doi = {10.1145/357103.357107},
  issn = {0164-0925},
  issue_date = {July 1980},
  numpages = {14},
  owner = {upuleegk},
  publisher = {ACM},
  timestamp = {2013.02.28},
  url = {http://doi.acm.org/10.1145/357103.357107}
}

@ARTICLE{Kelly201147,
  author = {Diane Kelly and Robert Gray and Yizhen Shao},
  title = {Examining random and designed tests to detect code mistakes in scientific
	software},
  journal = {Journal of Computational Science},
  year = {2011},
  volume = {2},
  pages = {47 - 56},
  number = {1},
  doi = {10.1016/j.jocs.2010.12.002},
  issn = {1877-7503},
  keywords = {Software testing},
  owner = {upuleegk},
  timestamp = {2013.02.28},
  url = {http://www.sciencedirect.com/science/article/pii/S187775031000075X}
}

@ARTICLE{5228715,
  author = {Kelly, D. and Hook, D. and Sanders, R.},
  title = {Five Recommended Practices for Computational Scientists Who Write
	Software},
  journal = {Computing in Science Engineering},
  year = {2009},
  volume = {11},
  pages = {48 -53},
  number = {5},
  month = {sept.-oct. },
  doi = {10.1109/MCSE.2009.139},
  issn = {1521-9615},
  keywords = {Best practices;Computer architecture;Computer interfaces;Data structures;Guidelines;Lifting
	equipment;Military computing;Software testing;User interfaces;Writing;software
	engineering;computational scientist;handbook;software engineering
	practice;software engineering technique;scientific software;},
  owner = {upuleegk},
  timestamp = {2013.02.28}
}

@INPROCEEDINGS{KellyAssesing2008,
  author = {D. Kelly and R. Sanders},
  title = {Assessing the quality of scientific software},
  booktitle = {Proc of the First International Workshop on Software Engineering
	for Computational Science and Engineering},
  year = {2008},
  owner = {upuleegk},
  timestamp = {2013.02.06}
}

@ARTICLE{5999781,
  author = {Kelly, Diane and Smith, Spencer and Meng, Nicholas},
  title = {Software Engineering for Scientists},
  journal = {Computing in Science Engineering},
  year = {2011},
  volume = {13},
  pages = {7 -11},
  number = {5},
  month = {sept.-oct. },
  doi = {10.1109/MCSE.2011.86},
  issn = {1521-9615},
  keywords = {Computational modeling;Software engineering;System design and analysis;Software
	engineering;computational science;scientific software;software development
	process;software education;software testing;software tools;},
  owner = {upuleegk},
  timestamp = {2013.02.28}
}

@ARTICLE{5467013,
  author = {Kelly, D. and Thorsteinson, S. and Hook, D.},
  title = {Scientific Software Testing: Analysis with Four Dimensions},
  journal = {Software, IEEE},
  year = {2011},
  volume = {28},
  pages = {84 -90},
  number = {3},
  month = {may-june },
  doi = {10.1109/MS.2010.88},
  issn = {0740-7459},
  keywords = {Application software;Cultural differences;Software engineering;Software
	testing;System testing;Time to market;natural sciences computing;program
	testing;code execution inspection;process-driven testing;scientific
	software development;scientific software testing;software assessment;software
	design;software engineering;software systems;multidisciplinary team;scientific
	software;software testing;},
  owner = {upuleegk},
  timestamp = {2013.02.28}
}

@TECHREPORT{chinASurvey2007,
  author = {L.S. Chin, D.J. Worth, and C. Greenough},
  title = {A Survey of Software Testing Tools for
	
	Computational Science},
  institution = {Rutherford Appleton Laboratory},
  year = {2007},
  number = {RAL-TR-2007-010},
  address = {Software Engineering Group
	
	Computational Science \& Engineering Department
	
	Rutherford Appleton Laboratory
	
	Harwell Science and Innovation Campus
	
	Didcot
	
	Oxfordshire OX11 0QX},
  owner = {upuleegk},
  timestamp = {2013.02.08}
}

@ARTICLE{doi:10.1080/0952813X.2012.695443,
  author = {Lane, Peter C.R. and Gobet, Fernand},
  title = {A theory-driven testing methodology for developing scientific software},
  journal = {Journal of Experimental \& Theoretical Artificial Intelligence},
  year = {2012},
  volume = {24},
  pages = {421-456},
  number = {4},
  doi = {10.1080/0952813X.2012.695443},
  eprint = {http://www.tandfonline.com/doi/pdf/10.1080/0952813X.2012.695443},
  owner = {upuleegk},
  timestamp = {2013.02.28},
  url = {http://www.tandfonline.com/doi/abs/10.1080/0952813X.2012.695443}
}

@INPROCEEDINGS{4032272,
  author = {Mayer, J. and Guderlei, R.},
  title = {On Random Testing of Image Processing Applications},
  booktitle = {Quality Software, 2006. QSIC 2006. Sixth International Conference
	on},
  year = {2006},
  pages = {85 -92},
  month = {oct.},
  doi = {10.1109/QSIC.2006.45},
  issn = {1550-6002},
  keywords = {Automatic testing;Digital images;Euclidean distance;Genetic mutations;Gray-scale;Image
	analysis;Image processing;Pixel;Software quality;Software testing;image
	processing;program testing;program verification;random processes;transforms;Euclidean
	distance transform;image processing applications;metamorphic Testing;metamorphic
	relation;mutation analysis;random image generation;random models;random
	testing;testing oracle;Metamorphic Testing;Random Testing;test data
	selection;test evaluation;testing oracle;},
  owner = {upuleegk},
  timestamp = {2013.02.28}
}

@INCOLLECTION{meinkeALearning2010,
  author = {Meinke, Karl and Niu, Fei},
  title = {A Learning-Based Approach to Unit Testing of Numerical Software},
  booktitle = {Testing Software and Systems},
  publisher = {Springer Berlin Heidelberg},
  year = {2010},
  editor = {Petrenko, Alexandre and Simão, Adenilso and Maldonado, JoséCarlos},
  volume = {6435},
  series = {Lecture Notes in Computer Science},
  pages = {221-235},
  doi = {10.1007/978-3-642-16573-3_16},
  isbn = {978-3-642-16572-6},
  owner = {upuleegk},
  timestamp = {2013.02.28},
  url = {http://dx.doi.org/10.1007/978-3-642-16573-3_16}
}

@INBOOK{Morris_2008,
  title = {Some Lessons Learned Reviewing Scientific Code},
  year = {2008},
  author = {Morris, Chris},
  booktitle = {Proceedings of the International Conference on Software Engineering},
  owner = {upuleegk},
  timestamp = {2013.02.14},
  url = {http://www.cse.msstate.edu/~SECSE08/Papers/Morris.pdf}
}

@INPROCEEDINGS{5380863,
  author = {Morris, C. and Segal, J.},
  title = {Some Challenges Facing Scientific Software Developers: The Case of
	Molecular Biology},
  booktitle = {e-Science, 2009. e-Science '09. Fifth IEEE International Conference
	on},
  year = {2009},
  pages = {216 -222},
  month = {dec.},
  doi = {10.1109/e-Science.2009.38},
  keywords = {Aggregates;Biology computing;Computational biology;Computational modeling;Councils;Explosions;Laboratories;Open
	source software;Programming;Software maintenance;biology computing;software
	engineering;molecular biology;physical sciences;scientific software
	developers;end user development;infrastructure;life sciences;molecular
	biology;protein;scientific software;},
  owner = {upuleegk},
  timestamp = {2013.02.28}
}

@INPROCEEDINGS{Murphy:2007:PRT:1292414.1292425,
  author = {Murphy, Christian and Kaiser, Gail and Arias, Marta},
  title = {Parameterizing random test data according to equivalence classes},
  booktitle = {Proceedings of the 2nd international workshop on Random testing:
	co-located with the 22nd IEEE/ACM International Conference on Automated
	Software Engineering (ASE 2007)},
  year = {2007},
  series = {RT '07},
  pages = {38--41},
  address = {New York, NY, USA},
  publisher = {ACM},
  acmid = {1292425},
  doi = {10.1145/1292414.1292425},
  isbn = {978-1-59593-881-7},
  keywords = {random test data generation, software testing},
  location = {Atlanta, Georgia},
  numpages = {4},
  owner = {upuleegk},
  timestamp = {2013.03.01},
  url = {http://doi.acm.org/10.1145/1292414.1292425}
}

@INPROCEEDINGS{Murphy:2011:ETH:1987993.1988003,
  author = {Murphy, Christian and Raunak, M. S. and King, Andrew and Chen, Sanjian
	and Imbriano, Christopher and Kaiser, Gail and Lee, Insup and Sokolsky,
	Oleg and Clarke, Lori and Osterweil, Leon},
  title = {On effective testing of health care simulation software},
  booktitle = {Proceedings of the 3rd Workshop on Software Engineering in Health
	Care},
  year = {2011},
  series = {SEHC '11},
  pages = {40--47},
  address = {New York, NY, USA},
  publisher = {ACM},
  acmid = {1988003},
  doi = {10.1145/1987993.1988003},
  isbn = {978-1-4503-0585-3},
  keywords = {metamorphic testing, oracle problem, software testing},
  location = {Waikiki, Honolulu, HI, USA},
  numpages = {8},
  owner = {upuleegk},
  timestamp = {2013.03.01},
  url = {http://doi.acm.org/10.1145/1987993.1988003}
}

@INPROCEEDINGS{Nguyen-Hoan:2010:SSS:1852786.1852802,
  author = {Nguyen-Hoan, Luke and Flint, Shayne and Sankaranarayana, Ramesh},
  title = {A survey of scientific software development},
  booktitle = {Proceedings of the 2010 ACM-IEEE International Symposium on Empirical
	Software Engineering and Measurement},
  year = {2010},
  series = {ESEM '10},
  pages = {12:1--12:10},
  address = {New York, NY, USA},
  publisher = {ACM},
  acmid = {1852802},
  articleno = {12},
  doi = {10.1145/1852786.1852802},
  isbn = {978-1-4503-0039-1},
  keywords = {scientific software, scientists, software engineering, survey},
  location = {Bolzano-Bozen, Italy},
  numpages = {10},
  owner = {upuleegk},
  timestamp = {2013.02.28},
  url = {http://doi.acm.org/10.1145/1852786.1852802}
}

@ARTICLE{SPE:SPE401,
  author = {Petty, Grant W.},
  title = {Automated computation and consistency checking of physical dimensions
	and units in scientific programs},
  journal = {Software: Practice and Experience},
  year = {2001},
  volume = {31},
  pages = {1067--1076},
  number = {11},
  doi = {10.1002/spe.401},
  issn = {1097-024X},
  keywords = {physical dimensions, units, scientific programming, Fortran 90},
  owner = {upuleegk},
  publisher = {John Wiley \& Sons, Ltd.},
  timestamp = {2013.02.15},
  url = {http://dx.doi.org/10.1002/spe.401}
}

@ARTICLE{gmd-5-1009-2012,
  author = {Pipitone, J. and Easterbrook, S.},
  title = {Assessing climate model software quality: a defect density analysis
	of three models},
  journal = {Geoscientific Model Development},
  year = {2012},
  volume = {5},
  pages = {1009--1022},
  number = {4},
  doi = {10.5194/gmd-5-1009-2012},
  owner = {upuleegk},
  timestamp = {2013.02.28},
  url = {http://www.geosci-model-dev.net/5/1009/2012/}
}

@ARTICLE{Pitt-Francis13092008,
  author = {Pitt-Francis, Joe and Bernabeu, Miguel O and Cooper, Jonathan and
	Garny, Alan and Momtahan, Lee and Osborne, James and Pathmanathan,
	Pras and Rodriguez, Blanca and Whiteley, Jonathan P and Gavaghan,
	David J},
  title = {Chaste: using agile programming techniques to develop computational
	biology software},
  journal = {Philosophical Transactions of the Royal Society A: Mathematical,
	Physical and Engineering Sciences},
  year = {2008},
  volume = {366},
  pages = {3111-3136},
  number = {1878},
  abstract = {Cardiac modelling is the area of physiome modelling where the available
	simulation software is perhaps most mature, and it therefore provides
	an excellent starting point for considering the software requirements
	for the wider physiome community. In this paper, we will begin by
	introducing some of the most advanced existing software packages
	for simulating cardiac electrical activity. We consider the software
	development methods used in producing codes of this type, and discuss
	their use of numerical algorithms, relative computational efficiency,
	usability, robustness and extensibility.We then go on to describe
	a class of software development methodologies known as test-driven
	agile methods and argue that such methods are more suitable for scientific
	software development than the traditional academic approaches. A
	case study is a project of our own, Cancer, Heart and Soft Tissue
	Environment, which is a library of computational biology software
	that began as an experiment in the use of agile programming methods.
	We present our experiences with a review of our progress thus far,
	focusing on the advantages and disadvantages of this new approach
	compared with the development methods used in some existing packages.We
	conclude by considering whether the likely wider needs of the cardiac
	modelling community are currently being met and suggest that, in
	order to respond effectively to changing requirements, it is essential
	that these codes should be more malleable. Such codes will allow
	for reliable extensions to include both detailed mathematical models—of
	the heart and other organs—and more efficient numerical techniques
	that are currently being developed by many research groups worldwide.},
  doi = {10.1098/rsta.2008.0096},
  eprint = {http://rsta.royalsocietypublishing.org/content/366/1878/3111.full.pdf+html},
  owner = {upuleegk},
  timestamp = {2013.02.28},
  url = {http://rsta.royalsocietypublishing.org/content/366/1878/3111.abstract}
}

@ARTICLE{Post:2004:SPM,
  author = {D. E. Post and R. P. Kendall},
  title = {Software Project Management and Quality Engineering Practices for
	Complex, Coupled Multiphysics, Massively Parallel Computational Simulations:
	Lessons Learned From {ASCI}},
  journal = j-IJHPCA,
  year = {2004},
  volume = {18},
  pages = {399--416},
  number = {4},
  month = {Winter},
  acknowledgement = {#ack-nhfb#},
  bibdate = {Tue Aug 31 09:59:45 MDT 2010},
  bibsource = {http://hpc.sagepub.com/content/18/4.toc; http://hpc.sagepub.com/content/by/year;
	http://www.math.utah.edu/pub/tex/bib/ijsa.bib},
  coden = {IHPCFL},
  doi = {http://dx.doi.org/10.1177/1094342004048534},
  fjournal = {International Journal of High Performance Computing Applications},
  issn = {1094-3420 (print), 1741-2846 (electronic)},
  issn-l = {1094-3420},
  owner = {upuleegk},
  timestamp = {2013.02.28},
  url = {http://hpc.sagepub.com/content/18/4/399.full.pdf+html}
}

@ARTICLE{6086527,
  author = {Remmel, H. and Paech, B. and Bastian, P. and Engwer, C.},
  title = {System Testing a Scientific Framework Using a Regression-Test Environment},
  journal = {Computing in Science Engineering},
  year = {2012},
  volume = {14},
  pages = {38 -45},
  number = {2},
  month = {march-april },
  doi = {10.1109/MCSE.2011.115},
  issn = {1521-9615},
  keywords = {Computational modeling;Object recognition;distributed processing;program
	testing;regression analysis;DUNE;complex scientific framework;distributed-and-unified
	numerics environment;regression-test environment;software product
	line engineering;system testing;variability modeling;Test execution;methods
	for SQA;methods for verification and validation;scientific computing;},
  owner = {upuleegk},
  timestamp = {2013.02.28}
}

@INPROCEEDINGS{5439,
  author = {Reupke, W.A. and Srinivasan, E. and Rigterink, P.V. and Card, D.N.},
  title = {The need for a rigorous development and testing methodology for medical
	software},
  booktitle = {Engineering of Computer-Based Medical Systems, 1988., Proceedings
	of the Symposium on the},
  year = {1988},
  pages = {15 -20},
  month = {jun},
  doi = {10.1109/ECBS.1988.5439},
  keywords = {Biomedical engineering;Biomedical imaging;Costs;Medical tests;Programming;Project
	management;Software quality;Software safety;Software systems;Software
	testing;medical administrative data processing;program testing;medical
	software development;medical software testing;product assurance;project
	management;prototyping;software engineering;},
  owner = {upuleegk},
  timestamp = {2013.02.28}
}

@ARTICLE{4548404,
  author = {Sanders, R. and Kelly, D.},
  title = {Dealing with Risk in Scientific Software Development},
  journal = {Software, IEEE},
  year = {2008},
  volume = {25},
  pages = {21 -28},
  number = {4},
  month = {july-aug. },
  doi = {10.1109/MS.2008.84},
  issn = {0740-7459},
  keywords = {Application software;Bridges;Chemistry;Defense industry;Educational
	institutions;Military computing;Optical computing;Physics computing;Programming;Risk
	management;natural sciences computing;program testing;risk management;software
	development management;system documentation;risk management;scientific
	software development;software engineering;software testing;system
	documentation;Professional end-user developer;empirical study;scientific
	application software;software development;software testing;},
  owner = {upuleegk},
  timestamp = {2013.02.28}
}

@INPROCEEDINGS{sanders08challenge,
  author = {Rebecca Sanders and Diane Kelly},
  title = {The Challenge of Testing Scientific Software},
  booktitle = {Proceedings Conference for the Association for Software Testing (CAST)},
  year = {2008},
  pages = {30-36},
  address = {Toronto},
  month = {July},
  owner = {upulee},
  timestamp = {2012.03.22}
}

@INPROCEEDINGS{5069156,
  author = {Segal, J.},
  title = {Some challenges facing software engineers developing software for
	scientists},
  booktitle = {Software Engineering for Computational Science and Engineering, 2009.
	SECSE '09. ICSE Workshop on},
  year = {2009},
  pages = {9 -14},
  month = {may},
  doi = {10.1109/SECSE.2009.5069156},
  keywords = {Biological information theory;Biological system modeling;Context modeling;Design
	engineering;High performance computing;Pressing;Production;Programming;Software
	prototyping;Software quality;natural sciences computing;software
	engineering;scientific software development;software engineering;user
	engagement;},
  owner = {upuleegk},
  timestamp = {2013.02.28}
}

@INPROCEEDINGS{,
  author = {J. Segal},
  title = {Models of Scientific Software Development},
  booktitle = {2008 Workshop Software Eng. in Computational Science and Eng. (SECSE
	08)},
  year = {2008},
  owner = {upuleegk},
  timestamp = {2012.02.28}
}

@ARTICLE{segalWhenSoftware2005,
  author = {Segal, Judith},
  title = {When Software Engineers Met Research Scientists: A Case Study},
  journal = {Empirical Software Engineering},
  year = {2005},
  volume = {10},
  pages = {517-536},
  doi = {10.1007/s10664-005-3865-y},
  issn = {1382-3256},
  issue = {4},
  keywords = {Case study; software engineers; scientific software; agile methodologies;
	tailoring methodologies},
  language = {English},
  owner = {upuleegk},
  publisher = {Kluwer Academic Publishers},
  timestamp = {2013.02.28},
  url = {http://dx.doi.org/10.1007/s10664-005-3865-y}
}

@INPROCEEDINGS{Sletholt:2011:LRA:1985782.1985784,
  author = {Sletholt, Magnus Thorstein and Hannay, Jo and Pfahl, Dietmar and
	Benestad, Hans Christian and Langtangen, Hans Petter},
  title = {A literature review of agile practices and their effects in scientific
	software development},
  booktitle = {Proceedings of the 4th International Workshop on Software Engineering
	for Computational Science and Engineering},
  year = {2011},
  series = {SECSE '11},
  pages = {1--9},
  address = {New York, NY, USA},
  publisher = {ACM},
  acmid = {1985784},
  doi = {10.1145/1985782.1985784},
  isbn = {978-1-4503-0598-3},
  keywords = {agile software development, literature review, scientific software,
	scrum, xp},
  location = {Waikiki, Honolulu, HI, USA},
  numpages = {9},
  owner = {upuleegk},
  timestamp = {2013.02.28},
  url = {http://doi.acm.org/10.1145/1985782.1985784}
}

@INCOLLECTION{smithATest2007,
  author = {Smith, BrianT.},
  title = {A Test Harness TH for Numerical Applications and Libraries},
  booktitle = {Grid-Based Problem Solving Environments},
  publisher = {Springer US},
  year = {2007},
  editor = {Gaffney, PatrickW. and Pool, JamesC.T.},
  volume = {239},
  series = {IFIP The International Federation for Information Processing},
  pages = {227-241},
  doi = {10.1007/978-0-387-73659-4_13},
  isbn = {978-0-387-73658-7},
  language = {English},
  owner = {upuleegk},
  timestamp = {2013.02.28},
  url = {http://dx.doi.org/10.1007/978-0-387-73659-4_13}
}

@INPROCEEDINGS{2004SPIE.5423..288S,
  author = {{Smith}, M.~C. and {Kelsey}, R.~L. and {Riese}, J.~M. and {Young},
	G.~A.},
  title = {{Creating a flexible environment for testing scientific software}},
  booktitle = {Society of Photo-Optical Instrumentation Engineers (SPIE) Conference
	Series},
  year = {2004},
  editor = {{Trevisani}, D.~A. and {Sisti}, A.~F.},
  volume = {5423},
  series = {Society of Photo-Optical Instrumentation Engineers (SPIE) Conference
	Series},
  pages = {288-296},
  month = aug,
  adsnote = {Provided by the SAO/NASA Astrophysics Data System},
  adsurl = {http://adsabs.harvard.edu/abs/2004SPIE.5423..288S},
  doi = {10.1117/12.542345},
  owner = {upuleegk},
  timestamp = {2013.02.28}
}

@ARTICLE{764216,
  author = {Stevenson, D.E.},
  title = {A critical look at quality in large-scale simulations},
  journal = {Computing in Science Engineering},
  year = {1999},
  volume = {1},
  pages = {53 -63},
  number = {3},
  month = {may/jun},
  doi = {10.1109/5992.764216},
  issn = {1521-9615},
  keywords = {ASCI management;ASCI science;large-scale simulations;simulation quality;software
	engineering;validation;digital simulation;program verification;software
	development management;software quality;},
  owner = {upuleegk},
  timestamp = {2013.02.28}
}

@INPROCEEDINGS{Tang:2010:PNC:1831708.1831724,
  author = {Tang, Enyi and Barr, Earl and Li, Xuandong and Su, Zhendong},
  title = {Perturbing numerical calculations for statistical analysis of floating-point
	program (in)stability},
  booktitle = {Proceedings of the 19th international symposium on Software testing
	and analysis},
  year = {2010},
  series = {ISSTA '10},
  pages = {131--142},
  address = {New York, NY, USA},
  publisher = {ACM},
  acmid = {1831724},
  doi = {10.1145/1831708.1831724},
  isbn = {978-1-60558-823-0},
  keywords = {floating-point, numerical code, perturbation, stability, testing},
  location = {Trento, Italy},
  numpages = {12},
  owner = {upuleegk},
  timestamp = {2013.02.28},
  url = {http://doi.acm.org/10.1145/1831708.1831724}
}

@INCOLLECTION{vilkomirModeling2008,
  author = {Vilkomir, SergiyA. and Swain, W.Thomas and Poore, JesseH. and Clarno,
	KevinT.},
  title = {Modeling Input Space for Testing Scientific Computational Software:
	A Case Study},
  booktitle = {Computational Science – ICCS 2008},
  publisher = {Springer Berlin Heidelberg},
  year = {2008},
  editor = {Bubak, Marian and Albada, GeertDick and Dongarra, Jack and Sloot,
	PeterM.A.},
  volume = {5103},
  series = {Lecture Notes in Computer Science},
  pages = {291-300},
  doi = {10.1007/978-3-540-69389-5_34},
  isbn = {978-3-540-69388-8},
  owner = {upuleegk},
  timestamp = {2013.02.28},
  url = {http://dx.doi.org/10.1007/978-3-540-69389-5_34}
}

@ARTICLE{Weyuker01111982,
  author = {Weyuker, Elaine J.},
  title = {On Testing Non-Testable Programs},
  journal = {The Computer Journal},
  year = {1982},
  volume = {25},
  pages = {465-470},
  number = {4},
  abstract = {A frequently invoked assumption in program testing is that there is
	an oracle (i.e. the tester or an external mechanism can accurately
	decide whether or not the output produced by a program is correct).
	A program is non-testable if either an oracle does not exist or the
	tester must expend some extraordinary amount of time to determine
	whether or not the output is correct. The reasonableness of the oracle
	assumption is examined and the conclusion is reached that in many
	cases this is not a realistic assumption. The consequences of assuming
	the availability of an oracle are examined and alternatives investigated.},
  doi = {10.1093/comjnl/25.4.465},
  eprint = {http://comjnl.oxfordjournals.org/content/25/4/465.full.pdf+html},
  owner = {upuleegk},
  timestamp = {2013.02.28},
  url = {http://comjnl.oxfordjournals.org/content/25/4/465.abstract}
}

@comment{jabref-meta: selector_review:}

@comment{jabref-meta: selector_publisher:}

@comment{jabref-meta: selector_author:}

@comment{jabref-meta: selector_journal:}

@comment{jabref-meta: selector_keywords:}


